Characteristic Spatial Scales in Earthquake Data

We present a new technique in order to quantify the dynamics of spatially extended systems. Using a test on the existence of unstable periodic orbits, we identify intermediate spatial scales, wherein the dynamics is characterized by maximum nontrivial determinism. This method is applied to earthquake catalogues containing time, coordinates and magnitude. As a result we extract a set of areas with significant deterministic and low-dimensional dynamics from the data. Finally, a simple model is used to show that these scales can be interpreted as local spatial coupling strengths.

==> wideabs <==
%auto-ignore

  You can actually get a first page that looks something like the first
page of Phys. Rev. (with abstract across the page), IF you are using
version 3.1 of REVTeX. Here is the general format:

\wideabs{
\title{ . . . }
   .
   .
   .
\pacs{ . . . }
}

That is, just insert the command \wideabs the title, and put the
ending curly brace after the pacs.

  Note that these lines should never appear in a file destined for the APS.
Note also that this is a quick hack and may have unknown drawbacks, along
with these known ones:

  (1) Byline footnotes (any footnotes or \thanks between the inserted lines)
      will probably just disappear.
  (2) No catcode changes can be effected between the inserted lines;
      mainly this means no verbatim and \verb, but may have other
      consequences.
It was intended to produce a style that had the abstract printed on the
width of the page, but there were always problems with the implementation and
so it was withdrawn near the release date. It may be possible to solve this
problem in the future.





